Security Science (SecSci), Basic Concepts and Mathematical Foundations

This textbook compiles the lecture notes from security courses taught at Oxford in the 2000s, at Royal Holloway in the 2010s, and currently in Hawaii. The early chapters are suitable for a first course in security. The middle chapters have been used in advanced courses. Towards the end there are also some research problems.

==> SecSci-macros.tex <==
% !TEX root = 000-SecSci.tex

% \usepackage{etex}
% per latex warning suggestion changed to:
\RequirePackage{etex}


%\usepackage{draftwatermark}
%\SetWatermarkText{{\tt 20250410 Peter's arxiv version}}
%\SetWatermarkScale{1}
%\SetWatermarkFontSize{.8cm}
%\SetWatermarkAngle{90}
%\SetWatermarkHorCenter{1.3cm}
%%\SetWatermarkVerCenter{.5cm}
%%\SetWatermarkColor[rgb]{0.8,0,0.1}
%\SetWatermarkColor[gray]{0.6}

\usepackage[utf8]{inputenc}
\usepackage[english]{babel}

%\usepackage[T2A,T1]{fontenc}
%\DeclareSymbolFont{cyrillic}{T2A}{cmr}{m}{n}
%\DeclareMathSymbol{\Sha}{\mathalpha}{cyrillic}{216}
%\DeclareMathSymbol{\sha}{\mathalpha}{cyrillic}{248}
%

\usepackage[makeindex,useindex]{splitidx}
%\makeindex
\usepackage{showidx}

%%% FORMATS

\usepackage{setspace}
\setlength{\parskip}{.75\baselineskip}
\setlength{\parindent}{0em}

%%\setlength{\parskip}{-.5\baselineskip}
%\setlength{\topsep}{.5\baselineskip}
%%\renewcommand{\baselinestretch}{1.15}

%%% PACKAGES
\usepackage{tikz}
\usetikzlibrary{cd,automata,arrows,positioning,decorations.pathreplacing,calc}


%\usepackage{tikz-cd}
\tikzcdset{
  shift left/.default=+0.7ex,% default: +0.56ex
  shift right/.default=+0.7ex}
\newenvironment{tikzar}[1][]{{}\kern-4pt\begin{tikzcd}[ampersand replacement=\&,#1]}%
{\end{tikzcd}\kern-4pt{}}
\tikzstyle{edge label%every node
}=[font=\scriptsize]
\tikzcdset{every label/.append style = {font = \scriptsize}}
\tikzcdset{every node/.append style = {font = \scriptsize}}

%\usepackage{txfonts}
\usepackage{graphicx}
\usepackage{pgf}

\usepackage{multicol}
\usepackage{multirow}
\usepackage{hhline}
\usepackage{array}
\newcolumntype{L}[1]{>{\raggedright\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{C}[1]{>{\centering\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{R}[1]{>{\raggedleft\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}

\usepackage{rotating}

\usepackage{pst-plot}
\usepackage{pstricks}

\usepackage{array}
\usepackage{multirow}

\usepackage{wrapfig}


\usepackage[LGR,T1]{fontenc}
\newcommand{\textgreek}[1]{\begingroup\fontencoding{LGR}\selectfont#1\endgroup}


% \usepackage{algorithmicx}
\usepackage{algpseudocode}

\algdef{SE}[ACTION]{Action}{EndAction}%
[2]{\algorithmicprocedure\ \textproc{#1}\ifthenelse{\equal{#2}{}}{}{(#2)}}%
{\algorithmicend\ \algorithmicaction}%

\algdef{SE}[COMMAND]{Command}{EndCommand}%
[2]{\algorithmicprocedure\ \textproc{#1}\ifthenelse{\equal{#2}{}}{}{(#2)}}%
{\algorithmicend\ \algorithmiccommand}%

\usepackage{amsfonts,amssymb,amsmath,amsthm}
\usepackage{stmaryrd}
\usepackage{txfonts}
%\usepackage{amsfonts,amssymb,amsmath,amsthm}
%\usepackage{stmaryrd}
\usepackage{fancybox,graphics,latexsym}
\usepackage{yfonts}
\newfont{\gothic}{ygoth at 12pt}



\theoremstyle{plain}
\newtheorem{theorem}{Theorem}[chapter]
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{example}[theorem]{Example}
\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\theoremstyle{remark}
\newtheorem*{remark}{Remark}


\usepackage{fullpage}
\usepackage{pgf}
% \usepackage{graphicx}
\usepackage{enumerate}

\usepackage{pstricks}

\makeatletter
\DeclareOldFontCommand{\rm}{\normalfont\rmfamily}{\mathrm}
\DeclareOldFontCommand{\sf}{\normalfont\sffamily}{\mathsf}
\DeclareOldFontCommand{\tt}{\normalfont\ttfamily}{\mathtt}
\DeclareOldFontCommand{\bf}{\normalfont\bfseries}{\mathbf}
\DeclareOldFontCommand{\it}{\normalfont\itshape}{\mathit}
\DeclareOldFontCommand{\sl}{\normalfont\slshape}{\@nomath\sl}
\DeclareOldFontCommand{\sc}{\normalfont\scshape}{\@nomath\sc}
\makeatother

%%% TABLEOFCONTENTS

%\usepackage{minitoc}
%\setcounter{minitocdepth}{3}    % Show subsubsections
%\dominitoc[n]      % [n] removes the title "Contents", [c] centers


%\usepackage{blindtext}
%\newcommand{\summary}[1]{
%\addtocontents{toc}{%\protect\vspace{-1.0em plus -1pt}
%}%
%%}{}
%\addtocontents{toc}{\textit{#1}}}

%\usepackage{etoolbox}
%\newcommand*{\lastlevel}{chapter}
%\pretocmd{\section}{\def\lastlevel{chapter}}{}{}
%\pretocmd{\subsection}{\def\lastlevel{subsection}}{}{}
%\pretocmd{\subsubsection}{\def\lastlevel{subsubsection}}{}{}
%
%\makeatletter
%\newcommand{\l@summary}[2]{%
%  \begingroup
%    \let\@dotsep\@M
%    \csname l@#2\endcsname{#1}{}%
%  \endgroup
%}
%
%\newcommand{\summary}[1]{%
%  \ifdefstring{\lastlevel}{chapter}{%
%    \addtocontents{toc}{\protect\vspace{-1.0em plus -1pt}}%
%  }{}%
%  \addtocontents{toc}{%
%    \protect\contentsline{summary}{\protect\numberline{}\normalfont\itshape
%  #1}{\lastlevel}}%
%}
%\makeatother
%
%\usepackage{pagenote}
%\makepagenote
%%\usepackage{enotez} % for endnotes
%%\usepackage{subcaption}
%
%\usepackage{etoolbox}
%\newcommand*{\lastlevel}{section}
%\pretocmd{\section}{\def\lastlevel{section}}{}{}
%\pretocmd{\subsection}{\def\lastlevel{subsection}}{}{}
%\pretocmd{\subsubsection}{\def\lastlevel{subsubsection}}{}{}
%
%\makeatletter
%\newcommand{\l@summary}[2]{%
%  \begingroup
%    \let\@dotsep\@M
%    \csname l@#2\endcsname{#1}{}%
%  \endgroup
%}
%
%\newcommand{\summary}[1]{%
%  \ifdefstring{\lastlevel}{section}{%
%    %\addtocontents{toc}{\protect\vspace{-1.0em plus -1pt}}%
%  }{}%
%  \addtocontents{toc}{%
%    \protect\contentsline{summary}{\protect\numberline{}\normalfont\itshape
%  #1}{\lastlevel}}%
%}
%\makeatother

\setcounter{secnumdepth}{4}
\setcounter{tocdepth}{5}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%% MINITOC

\providecommand*{\Ifstr}{\ifstr}% added because of changes in upcoming KOMA-Script version 3.28 and \ifstr replaced by \Ifstr in the code (see https://komascript.de/faq_deprecatedif) 
\usepackage{blindtext}
\usepackage{xcolor}
%\usepackage[usenames]{color}
\definecolor{lightBlue}{rgb}{.55,.55,1}
\definecolor{lightRed}{rgb}{1,.55,.55}

\usepackage{scrwfile}% avoid trouble with the limited number of write handles
\usepackage{xpatch}

\colorlet{partcolor}{blue}
\addtokomafont{partprefix}{\color{partcolor}}% change color of part prefix
\addtokomafont{part}{\normalcolor}% use normal color for part title
%\renewcommand*\partformat{\partname~\thepart}% if you want to remove \autodot from the definition
\RedeclareSectionCommand[
  tocdynnumwidth=true,%
  tocbeforeskip=1em%,
%  tocindent=1.5em
]{part}
\RedeclareSectionCommand[
  beforeskip=0pt,
  afterindent=false,
  afterskip=2\baselineskip,
  tocdynnumwidth,
  tocbeforeskip=1em plus 1pt minus 1pt,% add some glue
  toclinefill=\TOCLineLeaderFill,
    tocindent=1.5em
]{chapter}
\RedeclareSectionCommand[
  beforeskip=\baselineskip,
  afterindent=false,
  afterskip=.5\baselineskip,
  tocindent=1.5em,
  tocnumwidth=3.5em
]{section}
\RedeclareSectionCommand[
  beforeskip=.75\baselineskip,
  afterindent=false,
  afterskip=.5\baselineskip,
  tocindent=3.8em,
  tocnumwidth=4em
]{subsection}
\RedeclareSectionCommand[
  beforeskip=.5\baselineskip,
  afterindent=false,
  afterskip=.25\baselineskip,
  tocindent=7em,
  tocnumwidth=4.1em
]{subsubsection}
\RedeclareSectionCommand[
  tocindent=10em,
  tocnumwidth=5em
]{paragraph}
\RedeclareSectionCommand[
  tocindent=12em,
  tocnumwidth=6em
]{subparagraph}

\RedeclareSectionCommands
  [tocpagenumberwidth=3em]
  {part,chapter,section,subsection,paragraph,subparagraph}

% https://tex.stackexchange.com/a/359758
% https://tex.stackexchange.com/a/502077
\makeatletter
\newif\ifuseparttoc
\newcommand*{\parttoc}[1][\thepart]{% new command to generate and show a chapter toc
  \useparttoctrue% switch on part-toc-entries
  \edef\ext@parttoc{tcp#1}% extension of the part-toc-file, e.g., tcpI
  \DeclareNewTOC[
    listname=Contents,
    %unset=onecolumn% if the part toc should use twocolumn
  ]{\ext@parttoc}% declare a new toc file
  \begingroup
    \value{tocdepth}=\chaptertocdepth% we want entries down to chapter
    \listoftoc{\ext@parttoc}% show the toc with header
  \endgroup
}
\xapptocmd\addtocentrydefault{% patch the KOMA-Script's generic toc entry generator
  \ifuseparttoc% if part toc entries should be generated
    \expandafter\tocbasic@addxcontentsline\expandafter{\ext@parttoc}{#1}{#2}{#3}% do it
  \fi
}{}{}
\xpretocmd\part{\useparttocfalse}{}{}% entries in part toc are automatically switched off at start of \part
\newif\ifusechaptertoc% Switch to tell \addtocentrydefault to not only make entries to the toc-file but also to the current section-toc-file
\newcommand*{\chaptertoc}[2][\thechapter]{% new command to generate and show a chapter toc
  \usechaptertoctrue% switch on chapter-toc-entries
  \edef\ext@chaptoc{tcc#1}% extension of the chapter-toc-file, e.g., tcc1
  \DeclareNewTOC{\ext@chaptoc}% declare a new toc file
  %\addsec*{Contents}% header of the chaptertoc
  \setchapterpreamble{%
    \begin{minipage}{\linewidth}
      \hrulefill\par
      \value{tocdepth}=\subsectiontocdepth% we want entries down to subsection --- say \subsubsectiontocdepth if you want subsubsections 
      \listoftoc*{\ext@chaptoc}% show the toc without header
    \end{minipage}%
    \par\bigskip\nobreak\noindent\hrulefill\par
    \bigskip\noindent\ignorespaces% add some vertical space after the toc and do not indent the following text
  }%
}
\xapptocmd\addtocentrydefault{% patch the KOMA-Script's generic toc entry generator
  \ifusechaptertoc% if chapter toc entries should be generated
    \Ifstr{#1}{chapter}{}
      {\expandafter\tocbasic@addxcontentsline\expandafter{\ext@chaptoc}{#1}{#2}{#3}}% do it
  \fi
}{}{}
\xpretocmd\chapter{\usechaptertocfalse}{}{}% entries in chapter toc are automatically switched off at start of \chapter
\xpretocmd\part{\usechaptertocfalse}{}{}% entries in chapter toc are automatically switched off at start of \part
\makeatother

\newcommand\setchaptertoc[1][]{%
  \Ifstr{#1}{}
    {\AddtoOneTimeDoHook{heading/preinit/chapter}{\chaptertoc}}
    {\AddtoOneTimeDoHook{heading/preinit/chapter}{\chaptertoc[#1]}}%
}

\setcounter{tocdepth}{\chapternumdepth%\partnumdepth
}% depth of TOC

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\usepackage{minitoc}
%\setcounter{minitocdepth}{4}    % Show subsubsections
%\dominitoc      

%\usepackage{pagenote}
%\makepagenote
%\usepackage{enotez} % for endnotes
\usepackage[dvips]{hyperref} % for hyperlinks
\usepackage[capitalize]{cleveref}

%\usepackage{minitoc}
%\setcounter{minitocdepth}{4}    % Show subsubsections
%\dominitoc      

\mathcode`\<="4268 %left delimiter
\mathcode`\>="5269 %right delimiter
\mathchardef\gt="313E %relation >
\mathchardef\lt="313C %relation <

\newcommand{\tagg}[1]{\tag{\sf{#1}}}
\renewcommand{\to}{\rightarrow}
\newcommand{\ot}{\leftarrow}
\newcommand{\tto}[1]{\xrightarrow{#1}}
\newcommand{\oot}[1]{\xleftarrow{#1}}
\newcommand{\ttto}[2]{\xrightarrow[#2]{#1}}
\newcommand{\ooot}[2]{\xleftarrow[#2]{#1}}

\newcommand{\truss}[2]{\underset{#2}{\stackrel{#1}{\longrightarrow}}}

\newcommand{\epi}{\twoheadrightarrow}
\newcommand{\epileft}{\twoheadleftarrow}
\newcommand{\mono}{\rightarrowtail}
\newcommand{\monoleft}{\lefttarrowtail}
\newcommand{\inclusion}{\hookrightarrow}
\newcommand{\inclusionleft}{\hookleftarrow}
\newcommand{\eepi}[1]{\stackrel{#1}{\epi}}
\newcommand{\eepileft}[1]{\stackrel{#1}{\epileft}}
\newcommand{\mmono}[1]{\stackrel{#1}{\mono}}
\newcommand{\mmonoleft}[1]{\stackrel{#1}{\monoleft}}
\newcommand{\iinclusion}[1]{\stackrel{#1}{\inclusion}}
\newcommand{\iinclusionleft}[1]{\stackrel{#1}{\inclusionleft}}

\newcommand{\toto}{\rightrightarrows}
\newcommand{\ttotto}[2]{\underset{#2}{\overset{#1}{\rightrightarrows}}}

\newcommand{\rel}{\multimap}%{dashrightarrow}

\renewcommand{\mapsfrom}{\mathrel{\reflectbox{\ensuremath{\mapsto}}}}
%\newcommand{\longmapsfrom}{\mathrel{\reflectbox{\ensuremath{\longmapsto}}}}
\newcommand{\pto}{\rightharpoonup}
\newcommand{\ppto}[1]{\stackrel{#1}\pto}
\newcommand{\pot}{\leftharpoonup}
\newcommand{\ppot}[1]{\stackrel{#1}\pot}

\newcommand{\mapsdown}{\hspace{-1ex}\raisebox{1.5ex}{\turnbox{-90}{$\mapsto$}}}
\renewcommand{\mmapsto}[1]{\stackrel{#1}{\longmapsto}}
\newcommand{\mmmapsto}[2]{\underset{#2}{\stackrel{#1}{\longmapsto}}}


%\newcommand{\xxp}[2]{\left[{#1},{#2}\right]}
%\newcommand{\xxpp}[2]{\xxp{{#1}^+}{#2}}

\newcommand{\enco}[1]{\widehat{#1}}
%\newcommand{\enco}[1]{\left\ulcorner{#1}\right\urcorner}
%\newcommand{\enc}[1]{\lceil{#1}\rceil}
\newcommand{\deco}[1]{\left\{{#1}\right\}}

\newcommand{\cons}{::}


\newcommand{\im}{{\rm im}}
\newcommand{\id}{{id}}



\newcommand{\AAA}{{\cal A}}
\newcommand{\BBB}{{\cal B}}
\newcommand{\CCC}{{\cal C}}
\newcommand{\DDD}{{\cal D}}
\newcommand{\EEE}{{\cal E}}
\newcommand{\FFF}{{\cal F}}
\newcommand{\GGG}{{\cal G}}
\newcommand{\HHH}{{\cal H}}
\newcommand{\III}{{\cal I}}
\newcommand{\JJJ}{{\cal J}}
\newcommand{\KKK}{{\cal K}}
\newcommand{\LLL}{{\cal L}}
\newcommand{\MMM}{{\cal M}}
\newcommand{\NNN}{{\cal N}}
\newcommand{\OOO}{{\cal O}}
\newcommand{\PPP}{{\cal P}}
\newcommand{\QQQ}{{\cal Q}}
\newcommand{\RRR}{{\cal R}}
\newcommand{\SSS}{{\cal S}}
\newcommand{\TTT}{{\cal T}}
\newcommand{\UUU}{{\cal U}}
\newcommand{\VVV}{{\cal V}}
\newcommand{\WWW}{{\cal W}}
\newcommand{\XXX}{{\cal X}}
\newcommand{\YYY}{{\cal Y}}
\newcommand{\ZZZ}{{\cal Z}}
\renewcommand{\Bbb}{\mathbb}
\newcommand{\AAa}{{\Bbb A}}
\newcommand{\BBb}{{\Bbb B}}
\newcommand{\CCc}{{\Bbb C}}
\newcommand{\DDd}{{\Bbb D}}
\newcommand{\EEe}{{\Bbb E}}
\newcommand{\FFf}{{\Bbb F}}
\newcommand{\GGg}{{\Bbb G}}
\newcommand{\HHh}{{\Bbb H}}
\newcommand{\IIi}{{\Bbb I}}
\newcommand{\JJj}{{\Bbb J}}
\newcommand{\KKk}{{\Bbb K}}
\newcommand{\LLl}{{\Bbb L}}
\newcommand{\MMm}{{\Bbb M}}
\newcommand{\NNn}{{\Bbb N}}
\newcommand{\OOo}{{\Bbb O}}
\newcommand{\PPp}{{\Bbb P}}
\newcommand{\QQq}{{\Bbb Q}}
\newcommand{\RRr}{{\Bbb R}}
\newcommand{\SSs}{{\Bbb S}}
\newcommand{\TTt}{{\Bbb T}}
\newcommand{\UUu}{{\Bbb U}}
\newcommand{\VVv}{{\Bbb V}}
\newcommand{\WWw}{{\Bbb W}}
\newcommand{\XXx}{{\Bbb X}}
\newcommand{\YYy}{{\Bbb Y}}
\newcommand{\ZZz}{{\Bbb Z}}

\newcommand{\WP}{\mbox{\large $\wp$}}
\newcommand{\WPP}[1]{\WP\left({#1}\right)}
\newcommand{\Dist}{\Delta}
\newcommand{\Distt}[1]{\Dist\left({#1}\right)}
\newcommand{\DS}{\DDD}
%\newcommand{\EX}{\EEE}
\newcommand{\Inp}{\XXX}
\newcommand{\Oup}{\YYY}
\newcommand{\Mnd}{T}



\newcommand{\mathbold}[1]{\mbox{\boldmath $#1$}}

\newcommand{\aaa}{\mathbf{a}}
\newcommand{\bbb}{\mathbf{b}}
\newcommand{\ccc}{\mathbf{c}}
\newcommand{\ddd}{\mathbf{d}}
\newcommand{\eee}{\mathbf{e}}
\newcommand{\fff}{\mathbf{f}}
\renewcommand{\ggg}{\mathbf{g}}
\newcommand{\hhh}{\mathbf{h}}
\newcommand{\iii}{\mathbf{i}}
\newcommand{\jjj}{\mathbf{j}}
\newcommand{\kkk}{\mathbf{k}}
\newcommand{\elll}{\mathbf{\ell}}
\newcommand{\mmm}{\mathbf{m}}
\newcommand{\nnn}{\mathbf{n}}
\newcommand{\ooo}{\mathbf{o}}
\newcommand{\ppp}{\mathbf{p}}
\newcommand{\qqq}{\mathbf{q}}
\newcommand{\rrr}{\mathbf{r}}
\newcommand{\sss}{\mathbf{s}}
\newcommand{\ttt}{\mathbf{t}}
\newcommand{\uuu}{\mathbf{u}}
\newcommand{\vvv}{\mathbf{v}}
\newcommand{\www}{\mathbf{w}}
\newcommand{\xxx}{\mathbf{x}}
\newcommand{\yyy}{\mathbf{y}}
\newcommand{\zzz}{\mathbf{z}}

\renewcommand{\vec}{\mathbf}

\newcommand{\AaA}{{\mathfrak A}}
\newcommand{\BbB}{{\mathfrak B}}
\newcommand{\CcC}{{\mathfrak C}}
\newcommand{\DdD}{{\mathfrak D}}
\newcommand{\EeE}{{\mathfrak E}}
\newcommand{\FfF}{{\mathfrak F}}
\newcommand{\GgG}{{\mathfrak G}}
\newcommand{\HhH}{{\mathfrak H}}
\newcommand{\IiI}{{\mathfrak I}}
\newcommand{\JjJ}{{\mathfrak J}}
\newcommand{\KkK}{{\mathfrak K}}
\newcommand{\LlL}{{\mathfrak L}}
\newcommand{\MmM}{{\mathfrak M}}
\newcommand{\NnN}{{\mathfrak N}}
\newcommand{\OoO}{{\mathfrak O}}
\newcommand{\PpP}{{\mathfrak P}}
\newcommand{\QqQ}{{\mathfrak Q}}
\newcommand{\RrR}{{\mathfrak R}}
\newcommand{\SsS}{{\mathfrak S}}
\newcommand{\TtT}{{\mathfrak T}}
\newcommand{\UuU}{{\mathfrak U}}
\newcommand{\VvV}{{\mathfrak V}}
\newcommand{\WwW}{{\mathfrak W}}
\newcommand{\XxX}{{\mathfrak X}}
\newcommand{\YyY}{{\mathfrak Y}}
\newcommand{\ZzZ}{{\mathfrak Z}}

\newcommand{\aaA}{{\mathfrak a}}
\newcommand{\bbB}{{\mathfrak b}}
\newcommand{\ccC}{{\mathfrak c}}
\newcommand{\ddD}{{\mathfrak d}}
\newcommand{\eeE}{{\mathfrak e}}
\newcommand{\ffF}{{\mathfrak f}}
\newcommand{\ggG}{{\mathfrak g}}
\newcommand{\hhH}{{\mathfrak h}}
\newcommand{\iiI}{{\mathfrak i}}
\newcommand{\jjJ}{{\mathfrak j}}
\newcommand{\kkK}{{\mathfrak k}}
\newcommand{\llL}{{\mathfrak l}}
\newcommand{\mmM}{{\mathfrak m}}
\newcommand{\nnN}{{\mathfrak n}}
\newcommand{\ooO}{{\mathfrak o}}
\newcommand{\ppP}{{\mathfrak p}}
\newcommand{\qqQ}{{\mathfrak q}}
\newcommand{\rrR}{{\mathfrak r}}
\newcommand{\ssS}{{\mathfrak s}}
\newcommand{\ttT}{{\mathfrak t}}
\newcommand{\uuU}{{\mathfrak u}}
\newcommand{\vvV}{{\mathfrak v}}
\newcommand{\wwW}{{\mathfrak w}}
\newcommand{\xxX}{{\mathfrak x}}
\newcommand{\yyY}{{\mathfrak y}}
\newcommand{\zzZ}{{\mathfrak z}}




%===========================================================================
%      P. TAYLOR'S "END OF PROOF BOX":
%
%
%  The complexity of the macro necessary to get a little box on the
%  right-hand-side at the end of a proof is amazing.  It really does
%  have to be this long!  Otherwise you're liable to get it at the
%  beginning of the next line, or even on the next page.
%
\def\pushright#1{{%              set up
   \parfillskip=0pt            % so \par doesnt push \square to left
   \widowpenalty=10000         % so we dont break the page before \square
   \displaywidowpenalty=10000  % ditto
   \finalhyphendemerits=0      % TeXbook exercise 14.32
  %
  %                 horizontal
   \leavevmode                 % \nobreak means lines not pages
   \unskip                     % remove previous space or glue
   \nobreak                    % don't break lines
   \hfil                       % ragged right if we spill over
   \penalty50                  % discouragement to do so
   \hskip.2em                  % ensure some space
   \null                       % anchor following \hfill
   \hfill                      % push \square to right
   {#1}                        % the end-of-proof mark (or whatever)
  %
  %                   vertical
   \par}}                      % build paragraph

% prefer proofs with statements, also space after
\def\qed{\pushright{$\boxempty$}\penalty-700 \smallskip}

\newenvironment{prf}[1]{\begin{trivlist} \item[{\bf ~Proof}#1.]}%
{\qed\end{trivlist}}

\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\bea}{\begin{eqnarray}}
\newcommand{\eea}{\end{eqnarray}}
\newcommand{\bear}{\begin{eqnarray*}}
\newcommand{\eear}{\end{eqnarray*}}
\newcommand{\bpr}{\begin{prf}{}}
\newcommand{\epr}{\end{prf}}
\newcommand{\bprf}[1]{\begin{prf}{#1}}
\newcommand{\eprf}{\end{prf}}

\newenvironment{itemizz}[1]{\begin{itemize}\addtolength{\itemsep}{#1\baselineskip}}%
{\end{itemize}}

% \input{prooftree}
%%%%%%%%%%%%%%%%%%%%%
%SYNTAX:
%%
%%      \prooftree
%%              hyp1            produces:
%%              hyp2
%%              hyp3            hyp1    hyp2    hyp3
%%      \justifies              -------------------- rulename
%%              concl                   concl
%%      \thickness=0.08em
%%      \shiftright 2em
%%      \using
%%              rulename
%%      \endprooftree
%%
%% where the hypotheses may be similar structures or just formulae.
%%
%% To get a vertical string of dots instead of the proof rule, do
%%
%%      \prooftree                      which produces:
%%              [hyp]
%%      \using                                  [hyp]
%%              name                              .
%%      \proofdotseparation=1.2ex                 .name
%%      \proofdotnumber=4                         .
%%      \leadsto                                  .
%%              concl                           concl
%%      \endprooftree
%%
%% Within a prooftree, \[ and \] may be used instead of \prooftree and
%% \endprooftree; this is not permitted at the outer level because it
%% conflicts with LaTeX. Also,
%%      \Justifies
%% produces a double line. In LaTeX you can use \begin{prooftree} and
%% \end{prootree} at the outer level (however this will not work for the inner
%% levels, but in any case why would you want to be so verbose?).
%%
%% All of of the keywords except \prooftree and \endprooftree are optional
%% and may appear in any order. They may also be combined in \newcommand's
%% eg "\def\Cut{\using\sf cut\thickness.08em\justifies}" with the abbreviation
%% "\prooftree hyp1 hyp2 \Cut \concl \endprooftree". This is recommended and
%% some standard abbreviations will be found at the end of this file.
%%
%% \thickness specifies the breadth of the rule in any units, although
%% font-relative units such as "ex" or "em" are preferable.
%% It may optionally be followed by "=".
%% \proofrulebreadth=.08em or \setlength\proofrulebreadth{.08em} may also be
%% used either in place of \thickness or globally; the default is 0.04em.
%% \proofdotseparation and \proofdotnumber control the size of the
%% string of dots
%%
%% If proof trees and formulae are mixed, some explicit spacing is needed,
%% but don't put anything to the left of the left-most (or the right of
%% the right-most) hypothesis, or put it in braces, because this will cause
%% the indentation to be lost.
%%
%% By default the conclusion is centered wrt the left-most and right-most
%% immediate hypotheses (not their proofs); \shiftright or \shiftleft moves
%% it relative to this position. (Not sure about this specification or how
%% it should affect spreading of proof tree.)
%
% global assignments to dimensions seem to have the effect of stretching
% diagrams horizontally.
%
%%==========================================================================

\def\introrule{{\cal I}}\def\elimrule{{\cal E}}%%
\def\andintro{\using{\land}\introrule\justifies}%%
\def\impelim{\using{\Rightarrow}\elimrule\justifies}%%
\def\allintro{\using{\forall}\introrule\justifies}%%
\def\allelim{\using{\forall}\elimrule\justifies}%%
\def\falseelim{\using{\bot}\elimrule\justifies}%%
\def\existsintro{\using{\exists}\introrule\justifies}%%

%% #1 is meant to be 1 or 2 for the first or second formula
\def\andelim#1{\using{\land}#1\elimrule\justifies}%%
\def\orintro#1{\using{\lor}#1\introrule\justifies}%%

%% #1 is meant to be a label corresponding to the discharged hypothesis/es
\def\impintro#1{\using{\Rightarrow}\introrule_{#1}\justifies}%%
\def\orelim#1{\using{\lor}\elimrule_{#1}\justifies}%%
\def\existselim#1{\using{\exists}\elimrule_{#1}\justifies}

%%==========================================================================

\newdimen\proofrulebreadth \proofrulebreadth=.05em
\newdimen\proofdotseparation \proofdotseparation=1.25ex
\newdimen\proofrulebaseline \proofrulebaseline=2ex
\newcount\proofdotnumber \proofdotnumber=3
\let\then\relax
\def\hfi{\hskip0pt plus.0001fil}
\mathchardef\squigto="3A3B
%
% flag where we are
\newif\ifinsideprooftree\insideprooftreefalse
\newif\ifonleftofproofrule\onleftofproofrulefalse
\newif\ifproofdots\proofdotsfalse
\newif\ifdoubleproof\doubleprooffalse
\let\wereinproofbit\relax
%
% dimensions and boxes of bits
\newdimen\shortenproofleft
\newdimen\shortenproofright
\newdimen\proofbelowshift
\newbox\proofabove
\newbox\proofbelow
\newbox\proofrulename
%
% miscellaneous commands for setting values
\def\shiftproofbelow{\let\next\relax\afterassignment\setshiftproofbelow\dimen0 }
\def\shiftproofbelowneg{\def\next{\multiply\dimen0 by-1 }%
\afterassignment\setshiftproofbelow\dimen0 }
\def\setshiftproofbelow{\next\proofbelowshift=\dimen0 }
\def\setproofrulebreadth{\proofrulebreadth}

%=============================================================================
\def\prooftree{% NESTED ZERO (\ifonleftofproofrule)
%
% first find out whether we're at the left-hand end of a proof rule
\ifnum  \lastpenalty=1
\then   \unpenalty
\else   \onleftofproofrulefalse
\fi
%
% some space on left (except if we're on left, and no infinity for outermost)
\ifonleftofproofrule
\else   \ifinsideprooftree
        \then   \hskip.5em plus1fil
        \fi
\fi
%
% begin our proof tree environment
\bgroup% NESTED ONE (\proofbelow, \proofrulename, \proofabove,
%               \shortenproofleft, \shortenproofright, \proofrulebreadth)
\setbox\proofbelow=\hbox{}\setbox\proofrulename=\hbox{}%
\let\justifies\proofover\let\leadsto\proofoverdots\let\Justifies\proofoverdbl
\let\using\proofusing\let\[\prooftree
\ifinsideprooftree\let\]\endprooftree\fi
\proofdotsfalse\doubleprooffalse
\let\thickness\setproofrulebreadth
\let\shiftright\shiftproofbelow \let\shift\shiftproofbelow
\let\shiftleft\shiftproofbelowneg
\let\ifwasinsideprooftree\ifinsideprooftree
\insideprooftreetrue
%
% now begin to set the top of the rule (definitions local to it)
\setbox\proofabove=\hbox\bgroup$\displaystyle % NESTED TWO
\let\wereinproofbit\prooftree
%
% these local variables will be copied out:
\shortenproofleft=0pt \shortenproofright=0pt \proofbelowshift=0pt
%
% flags to enable inner proof tree to detect if on left:
\onleftofproofruletrue\penalty1
}

%=============================================================================
% end whatever box and copy crucial values out of it
\def\eproofbit{% NESTED TWO
%
% various hacks applicable to hypothesis list 
\ifx    \wereinproofbit\prooftree
\then   \ifcase \lastpenalty
        \then   \shortenproofright=0pt  % 0: some other object, no indentation
        \or     \unpenalty\hfil         % 1: empty hypotheses, just glue
        \or     \unpenalty\unskip       % 2: just had a tree, remove glue
        \else   \shortenproofright=0pt  % eh?
        \fi
\fi
%
% pass out crucial values from scope
\global\dimen0=\shortenproofleft
\global\dimen1=\shortenproofright
\global\dimen2=\proofrulebreadth
\global\dimen3=\proofbelowshift
\global\dimen4=\proofdotseparation
\global\count255=\proofdotnumber
%
% end the box
$\egroup  % NESTED ONE
%
% restore the values
\shortenproofleft=\dimen0
\shortenproofright=\dimen1
\proofrulebreadth=\dimen2
\proofbelowshift=\dimen3
\proofdotseparation=\dimen4
\proofdotnumber=\count255
}

%=============================================================================
\def\proofover{% NESTED TWO
\eproofbit % NESTED ONE
\setbox\proofbelow=\hbox\bgroup % NESTED TWO
\let\wereinproofbit\proofover
$\displaystyle
}%
%
%=============================================================================
\def\proofoverdbl{% NESTED TWO
\eproofbit % NESTED ONE
\doubleprooftrue
\setbox\proofbelow=\hbox\bgroup % NESTED TWO
\let\wereinproofbit\proofoverdbl
$\displaystyle
}%
%
%=============================================================================
\def\proofoverdots{% NESTED TWO
\eproofbit % NESTED ONE
\proofdotstrue
\setbox\proofbelow=\hbox\bgroup % NESTED TWO
\let\wereinproofbit\proofoverdots
$\displaystyle
}%
%
%=============================================================================
\def\proofusing{% NESTED TWO
\eproofbit % NESTED ONE
\setbox\proofrulename=\hbox\bgroup % NESTED TWO
\let\wereinproofbit\proofusing
\kern0.3em$
}

%=============================================================================
\def\endprooftree{% NESTED TWO
\eproofbit % NESTED ONE
% \dimen0 =     length of proof rule
% \dimen1 =     indentation of conclusion wrt rule
% \dimen2 =     new \shortenproofleft, ie indentation of conclusion
% \dimen3 =     new \shortenproofright, ie
%                space on right of conclusion to end of tree
% \dimen4 =     space on right of conclusion below rule
  \dimen5 =0pt% spread of hypotheses
% \dimen6, \dimen7 = height & depth of rule
%
% length of rule needed by proof above
\dimen0=\wd\proofabove \advance\dimen0-\shortenproofleft
\advance\dimen0-\shortenproofright
%
% amount of spare space below
\dimen1=.5\dimen0 \advance\dimen1-.5\wd\proofbelow
\dimen4=\dimen1
\advance\dimen1\proofbelowshift \advance\dimen4-\proofbelowshift
%
% conclusion sticks out to left of immediate hypotheses
\ifdim  \dimen1<0pt
\then   \advance\shortenproofleft\dimen1
        \advance\dimen0-\dimen1
        \dimen1=0pt
%       now it sticks out to left of tree!
        \ifdim  \shortenproofleft<0pt
        \then   \setbox\proofabove=\hbox{%
                        \kern-\shortenproofleft\unhbox\proofabove}%
                \shortenproofleft=0pt
        \fi
\fi
%
% and to the right
\ifdim  \dimen4<0pt
\then   \advance\shortenproofright\dimen4
        \advance\dimen0-\dimen4
        \dimen4=0pt
\fi
%
% make sure enough space for label
\ifdim  \shortenproofright<\wd\proofrulename
\then   \shortenproofright=\wd\proofrulename
\fi
%
% calculate new indentations
\dimen2=\shortenproofleft \advance\dimen2 by\dimen1
\dimen3=\shortenproofright\advance\dimen3 by\dimen4
%
% make the rule or dots, with name attached
\ifproofdots
\then
        \dimen6=\shortenproofleft \advance\dimen6 .5\dimen0
        \setbox1=\vbox to\proofdotseparation{\vss\hbox{$\cdot$}\vss}%
        \setbox0=\hbox{%
                \advance\dimen6-.5\wd1
                \kern\dimen6
                $\vcenter to\proofdotnumber\proofdotseparation
                        {\leaders\box1\vfill}$%
                \unhbox\proofrulename}%
\else   \dimen6=\fontdimen22\the\textfont2 % height of maths axis
        \dimen7=\dimen6
        \advance\dimen6by.5\proofrulebreadth
        \advance\dimen7by-.5\proofrulebreadth
        \setbox0=\hbox{%
                \kern\shortenproofleft
                \ifdoubleproof
                \then   \hbox to\dimen0{%
                        $\mathsurround0pt\mathord=\mkern-6mu%
                        \cleaders\hbox{$\mkern-2mu=\mkern-2mu$}\hfill
                        \mkern-6mu\mathord=$}%
                \else   \vrule height\dimen6 depth-\dimen7 width\dimen0
                \fi
                \unhbox\proofrulename}%
        \ht0=\dimen6 \dp0=-\dimen7
\fi
%
% set up to centre outermost tree only
\let\doll\relax
\ifwasinsideprooftree
\then   \let\VBOX\vbox
\else   \ifmmode\else$\let\doll=$\fi
        \let\VBOX\vcenter
\fi
% this \vbox or \vcenter is the actual output:
\VBOX   {\baselineskip\proofrulebaseline \lineskip.2ex
        \expandafter\lineskiplimit\ifproofdots0ex\else-0.6ex\fi
        \hbox   spread\dimen5   {\hfi\unhbox\proofabove\hfi}%
        \hbox{\box0}%
        \hbox   {\kern\dimen2 \box\proofbelow}}\doll%
%
% pass new indentations out of scope
\global\dimen2=\dimen2
\global\dimen3=\dimen3
\egroup % NESTED ZERO
\ifonleftofproofrule
\then   \shortenproofleft=\dimen2
\fi
\shortenproofright=\dimen3
%
% some space on right and flag we've just made a tree
\onleftofproofrulefalse
\ifinsideprooftree
\then   \hskip.5em plus 1fil \penalty2
\fi
}
%%%%%%%%%%%%%%%%%%%%%

\usepackage{array}
\usepackage{multirow}

%% comment out duplicate definition ...
% \newcolumntype{L}[1]{>{\raggedright\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
% \newcolumntype{C}[1]{>{\centering\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
% \newcolumntype{R}[1]{>{\raggedleft\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}


\newcommand{\Act}{\AAa}%{\AAA}
\newcommand{\Actl}{\widehat{\Act}}%{\widehat{\AAA}}
\newcommand{\Levels}{\LLl}
\newcommand{\Event}{\Sigma}%{\EEE}
\newcommand{\Oper}{\Gamma}
\newcommand{\Subj}{\SSs}
\newcommand{\Role}{\RRr}
\newcommand{\Obj}{\JJj}
\newcommand{\subj}{subject }
\newcommand{\subjj}{subject}
\newcommand{\subjs}{subjects }
\newcommand{\subjss}{subjects}
\newcommand{\objj}{object}
\newcommand{\objss}{objects}
\newcommand{\obj}{object }
\newcommand{\objs}{objects }
\newcommand{\actt}{action}
\newcommand{\actss}{actions}

\newcommand{\suct}{\mathit{sbjt}}
\newcommand{\obct}{\mathit{objt}}
\newcommand{\actn}{\mathit{actn}}
\newcommand{\levl}{\mathit{levl}}



\newcommand{\AM}{B}
\newcommand{\AML}{\beta}
\newcommand{\PM}{M}
\newcommand{\PML}{\mu}
\newcommand{\States}{Q}
\newcommand{\Actions}{A}
\newcommand{\owner}{{\tt u}}
\newcommand{\group}{{\tt g}}
\newcommand{\others}{{\tt o}}
\newcommand{\clr}{c\ell}
\newcommand{\Clr}{C\ell}
\newcommand{\loc}{p\ell }
\newcommand{\locc}{p\ell}
%\newcommand{\clr}{\mathbf c}
%\newcommand{\loc}{\mathbf l}
\newcommand{\rd}{{r\hspace{-2.2ex}\searrow}}%{\tt r\hspace{-1.85ex}\searrow\,}%{\tt r}%{{\tt r}}
\newcommand{\rdd}{{\scriptstyle 
r\hspace{-1ex}\searrow}}%{\tt r\hspace{-1.85ex}\searrow\,}%{\tt r}%{{\tt r}}
\newcommand{\wt}{{w\hspace{-2.5ex}\nwarrow}}%{\tt w\hspace{-2.05ex}\nwarrow\,}%{\tt w}%{{\tt w}}
\newcommand{\wtt}{{\scriptstyle 
w\hspace{-1.2ex}\nwarrow}}%{\tt w\hspace{-2.05ex}\nwarrow\,}%{\tt w}%{{\tt w}}

\newcommand{\send}[1]{\left<\, #1\, \right>}
\newcommand{\recv}[1]{\left(\, #1\, \right)}
\newcommand{\ssend}[2]{\left<\, #1\, \right>_{#2}}
\newcommand{\rrecv}[2]{\left(\, #1\, \right)_{#2}}
%\newcommand{\qu}[2]{\left({#2}\!:\!{#1}?\right)}
%\newcommand{\an}[2]{\left({#2}\!:\!{#1}!\right)}
\newcommand{\qu}[2]{{#2}\!:\!{#1}?}
\newcommand{\an}[2]{{#2}\!:\!{#1}!}
\newcommand{\eqc}[1]{\left[\, #1\, \right]}



%%%%%% from 355-notes-macros.tex
\newcommand{\Guess}{G}
\newcommand{\CDH}{{\sf CDH}}
\newcommand{\DDH}{{\sf DDH}}
\newcommand{\order}{{\sf ord}}
\newcommand{\Keys}{\KKK}
\newcommand{\Msgs}{\MMM}
\newcommand{\Ciph}{\CCC}
\newcommand{\Code}{\GGG}
\newcommand{\Source}{\XXX}
\newcommand{\Seed}{\RRR}
\newcommand{\Gen}{{\sf K}}
\newcommand{\Enc}{{\sf E}}
\newcommand{\Genp}{{\KKk}}
\newcommand{\Encp}{{\EEe}}
\newcommand{\Dec}{{\sf D}}
\newcommand{\Att}{{\sf A}}%\mbox{\Large $\alpha$}}
\newcommand{\Attp}{{\AAa}}%\mbox{\Large $\alpha$}}
%\newcommand{\Sigs}{\SSS}
%\newcommand{\Sig}{{\sf S}}
%\newcommand{\Ver}{{\sf V}}
%
%\newcommand{\rar}{\triangleright}%{\shortrightarrow}
%\newcommand{\lal}{\triangleleft}%{\shortrightarrow}
%\newcommand{\lto}{\mbox{ to }}
%\newcommand{\sto}{\mbox{ \footnotesize to }}
%
%\newcommand{\blu}{\color{blue!50!black}}
%
%\newcommand{\from}{\!\in\!}%{\!\shortleftarrow\!}
\newcommand{\der}[1]{\ \underset{#1}{\mbox{\huge ${\vdash}$}}\ }
\renewcommand{\hom}[2]{\big[#1\ {\mbox{\large ${\vdash}$}}\ #2\big]}
%from LangEng
%\newcommand{\der}[2]{\ {#1}\ \ {\mbox{ \large ${\vdash}$}}\ \ {2}}
%\newcommand{\derr}[2]{\ \mbox{#1}\ {\mbox{\large ${\vdash}$}}\ \mbox{#2}}
%

%\newcommand{\hhom}[3]{\big[#1\ \stackrel{#2}{\vdash}\ {#3}\big]}
%\newcommand{\hhom}[3]{\big[#1\ \underset{#2}{\vdash}\ {#3}\big]}
\newcommand{\hhom}[3]{\big[#1\ {\vdash}_{#2}\ {#3}\big]}
\newcommand{\homm}[1]{\big[#1\big]}
\newcommand{\state}{\mathrm{St}}
%{\left[\begin{smallmatrix}\displaystyle #1 \end{smallmatrix}\right]}%

\newcommand{\pder}[2]{\big[#1\ {\mbox{\large ${\vdash}$}}\ #2\big]}
\newcommand{\ppder}[1]{\big[#1\big]}
\newcommand{\pderr}[2]{\big[\mbox{#1}\ {\mbox{\large ${\vdash}$}}\ \mbox{#2}\big]}
\newcommand{\ppderr}[1]{\big[\mbox{#1}\big]}



\renewcommand{\Pr}{\mathrm{Pr}}


%%%%%%%%%%%%%OLD 355 BEGIN%%%%%%%%%
%
%\newcommand{\Subj}{\SSS}
%\newcommand{\Obj}{\OOO}
%\newcommand{\Act}{\AAA}
%\newcommand{\Levels}{\LLl}
%\newcommand{\AM}{B}
%\newcommand{\PM}{M}
%\newcommand{\States}{Q}
%\newcommand{\Actions}{A}
%\newcommand{\owner}{{\mathbbm u}}
%\newcommand{\group}{{\mathbbm g}}
%\newcommand{\others}{{\mathbbm o}}
%\newcommand{\clr}{\mathbbm c}
%\newcommand{\loc}{\mathbbm l%\ell
%}
%\newcommand{\rd}{{\mathbbm r}}
%\newcommand{\wt}{{\mathbbm w}}
%
%\newcommand{\Guess}{G}
%\newcommand{\CDH}{{\sf CDH}}
%\newcommand{\DDH}{{\sf DDH}}
%\newcommand{\order}{{\sf ord}}
%\newcommand{\Keys}{\KKK}
%\newcommand{\Msgs}{\MMM}
%\newcommand{\Cyph}{\CCC}
%\newcommand{\Code}{\GGG}
%\newcommand{\Source}{\XXX}
%\newcommand{\Seed}{\RRR}
%\newcommand{\Gen}{{\sf K}}
%\newcommand{\Enc}{{\sf E}}
%\newcommand{\Genp}{{\KKk}}
%\newcommand{\Encp}{{\EEe}}
%\newcommand{\Dec}{{\sf D}}
%\newcommand{\Att}{{\sf A}}%\mbox{\Large $\alpha$}}
%\newcommand{\Attp}{{\AAa}}%\mbox{\Large $\alpha$}}
%\newcommand{\Sigs}{\SSS}
%\newcommand{\Sig}{{\sf S}}
%\newcommand{\Ver}{{\sf V}}
%
%%\newcommand{\rar}{\triangleright}%{\shortrightarrow}
%%\newcommand{\lal}{\triangleleft}%{\shortrightarrow}
%%\newcommand{\lto}{\mbox{ to }}
%%\newcommand{\sto}{\mbox{ \footnotesize to }}
%
%
%\newcommand{\blu}{\color{blue!50!black}}
%\newcommand{\tagg}[1]{\tag{\sf{#1}}}
%
%\newcommand{\from}{\!\in\!}%{\!\shortleftarrow\!}
%\newcommand{\der}[2]{\big(#1\, \vdash\, #2 \big)}
%\renewcommand{\hom}[2]{\big[#1\, \vdash\, #2\big]}
%%\renewcommand{\hom}[2]{\big[#1\ {\mbox{\LARGE ${\vdash}$}}\ #2\big]}
%\newcommand{\homm}[1]{\big[#1\big]}

\newcommand{\sta}{\varrho}
\newcommand{\lvl}{\boldmath c}

\newcommand{\out}{\delta}
\newcommand{\Out}{\partial}
\newcommand{\OUT}{d}

\newcommand{\Psb}{\WP^\bullet}
\newcommand{\Prb}{\Delta}
\newcommand{\In}{I}
\newcommand{\Ou}{J}
\newcommand{\St}{Q}



\newcommand{\prc}{\prec}
\newcommand{\auth}{\propto}
\newcommand{\compl}[1]{\neg{#1}}%{{#1}^c}
\newcommand{\halts}{\!\!\downarrow}
\newcommand{\domain}{\downarrow\!\!}
\newcommand{\restr}{\!\restriction}
\newcommand{\ineq}[1]{\left\lfloor{#1}\right\rfloor}%{\underset{#1}{\sim}}
\newcommand{\oueq}[1]{\left\lceil {#1}\right\rceil}%{\Rsh{#1}\Lsh}%{\underset{#1}{\approx}}

\newcommand{\direct}{direct}
\newcommand{\channel}{channel}
\newcommand{\oth}{\neg}

\newcommand{\lft}[1]{\protect\overleftarrow{#1}}
\newcommand{\rgt}[1]{\protect\overrightarrow{#1}}
\newcommand{\Lft}[1]{{\overset{\Longleftarrow}{#1}}}
\newcommand{\Rgt}[1]{{\overset{\Longrightarrow}{#1}}}

\newcommand{\cut}[1]{\protect\overleftrightarrow{#1}} 

\newcommand{\proj}{\Lambda}
\newcommand{\hd}{\rgt{\sf h}}%{\hhh.\!}
\newcommand{\ta}{\rgt{\sf t}}%{.\!\ttt}
\renewcommand{\dh}{\lft{\sf h}}%{.\!\hhh}
\newcommand{\at}{\lft{\sf t}}%{\ttt.\!}


\newcommand{\Lo}{{\rm Lo}}
\newcommand{\Hi}{{\rm Hi}}

\newcommand{\para}[1]{\noindent\textbf{\textsf{#1}}}



\newcommand{\Ent}{{\sf E}}
\newcommand{\SafE}{\mbox{\rm SafElev}}
\newcommand{\LivE}{\mbox{\rm LivElev}}
\newcommand{\SafC}{\mbox{\rm AskQ}}
\newcommand{\LivC}{\mbox{\rm AnsQ}}
\newcommand{\SAF}{{\sf Safe}}%{\SSS\AAA}
\newcommand{\LIV}{{\sf Live}}%{\LLL\III}
\newcommand{\AU}{{\sf Auth}}%{\AAA\UUU}
\newcommand{\AV}{{\sf Avail}}%{\AAA\VVV}
\newcommand{\WAV}{{\sf WAva}}
\newcommand{\SAV}{{\sf SAva}}%
\newcommand{\NAU}{{\sf NAut}}
\newcommand{\CRAU}{{\sf ChRe}}
\newcommand{\Local}{{\sf Loc}}
\newcommand{\Space}{E}\newcommand{\Cylout}{{\sf ExCyl}}
\newcommand{\Cylin}{{\sf InCyl}}\newcommand{\AuthoE}{\mbox{\rm AuthElev}}
\newcommand{\AvailE}{\mbox{\rm AvailElev}}
\newcommand{\AuthoC}{\mbox{\rm NoBadConv}}
\newcommand{\AvailC}{\mbox{\rm GoodConv}}

\newcommand{\Subsp}{{\sf W}}
\newcommand{\Closed}{F}
\newcommand{\Dense}{D}
\newcommand{\Property}{P}
\newcommand{\Service}{{\rm Service}}
\newcommand{\Qroperty}{P}
\newcommand{\Croperty}{\overline{P}}
\newcommand{\clos}[1]{c\left(#1\right)}
\newcommand{\bound}[1]{b\left(#1\right)}
\newcommand{\seq}[1]{\big(\, #1\, \big)}
\newcommand{\sseq}[1]{\left(\, #1\, \right)}

\newcommand{\length}[1]{\lvert {#1}\rvert}%{\left[\begin{smallmatrix}\displaystyle #1 \end{smallmatrix}\right]}%
\newcommand{\milk}{\mbox{milk}}
\newcommand{\schedule}{s}
\newcommand{\sschedule}{schedule}

\newcommand{\cata}[1]{\llparenthesis {#1} \rrparenthesis}
\newcommand{\ana}[1]{\left\llbracket {#1} \right\rrbracket}

\newcommand{\closure}[1]{\nabla{#1}}
\newcommand{\interior}[1]{\Delta{#1}}




\newcommand{\censure}{censure}

\newcommand{\functional}{{functional}}
\newcommand{\relational}{{relational}}
\newcommand{\stochastic}{{stochastic}}
\newcommand{\Relational}{{Relational}}
\newcommand{\Stochastic}{{Stochastic}}

\newcommand{\nice}{nice}
\newcommand{\Nice}{Nice}

\newcommand{\comme}{{\scriptstyle\rightsquigarrow}}%{\mbox{\footnotesize$\rightsquigarrow$}}
\newcommand{\sstay}{\odot}

\newcommand{\Prob}[1]{\Pr_{#1}}
\newcommand{\Probb}{{\rm Pr}}
\newcommand{\pxx}{\textit{past}}%{\textrm{prefix}}
\newcommand{\sxx}{\textit{last}}%{\textrm{suffix}}
\newcommand{\constr}{\textrm{constr}}
\newcommand{\destr}{\textrm{destr}}
\newcommand{\intt}{\textstyle{\int}}
\newcommand{\ladj}[1]{{#1}^{\ast}}
\newcommand{\radj}[1]{{#1}_{\ast}}


\newcommand{\bra}[1]{<{#1}\, |}\newcommand{\ket}[1]{|\, {#1}\,>}
\newcommand{\braa}[1]{<\mbox{#1}|}
\newcommand{\kett}[1]{|\,\mbox{#1}\,>}
\newcommand{\braket}[2]{<{#1}\, |\, {#2}>}
\newcommand{\brakett}[2]{<\mbox{#1}\, |\, \mbox{#2}>}
\newcommand{\brakem}[3]{<{#1}\, |\, {#2}\,|\, {#3}>}
\newcommand{\brakemm}[3]{<\mbox{#1}\, |\, \mbox{#2}\, |\, \mbox{#3}>}

\newcommand{\ccoin}{\includegraphics[height = 1.75ex]{coin.eps}}

%\newcommand{\cccoin}{\includegraphics[height = 1.75ex]{coin.eps}}

\newcommand{\blank}{\square}

%%%%%%%%%%%%%OLD 355 END%%%%%%%%%%%%



